SOFIA FEEDBACK survey: PDR diagnostics of stellar feedback in different regions of RCW 49

We quantified the effects of stellar feedback in RCW 49 by determining the physical conditions in different regions using the [CII] 158 $\mu$m and [OI] 63 $\mu$m observations from SOFIA, the $^{12}$CO (3-2) observations from APEX and the H$_2$ line observations from Spitzer telescopes. Large maps of RCW 49 were observed with the SOFIA and APEX telescopes, while the Spitzer observations were only available towards three small areas. From our qualitative analysis, we found that the H$_2$ 0-0 S(2) emission line probes denser gas compared to the H$_2$ 0-0 S(1) line. In four regions ("northern cloud", "pillar", "ridge", and "shell"), we compared our observations with the updated PDR Toolbox models and derived the integrated far-ultraviolet flux between 6-13.6 eV ($G_{\rm 0}$), H nucleus density ($n$), temperatures and pressures. We found the ridge to have the highest $G_{\rm 0}$ (2.4 $\times$ 10$^3$ Habing units), while the northern cloud has the lowest $G_{\rm 0}$ (5 $\times$ 10$^2$ Habing units). This is a direct consequence of the location of these regions with respect to the Wd2 cluster. The ridge also has a high density (6.4 $\times$ 10$^3$ cm$^{-3}$), which is consistent with its ongoing star formation. Among the Spitzer positions, we found the one closest to the Wd2 cluster to be the densest, suggesting an early phase of star formation. Furthermore, the Spitzer position that overlaps with the shell was found to have the highest $G_{\rm 0}$ and we expect this to be a result of its proximity to an O9V star.

==> table0.tex <==

\begin{deluxetable}{l c c}
%\tabletypesize{\footnotesize}
%\tablecolumns{8}
%\tablewidth{\textwidth}
\tablecaption{Interesting regions in RCW~49.}
\label{tab:regions-pos}
\tablehead{
\colhead{Region} & 
\colhead{R.A. (J2000)} & 
\colhead{Dec. (J2000)} 
}
\startdata
{northern cloud} & 10:23:59.733 & -57:38:52.74\\
ridge &10:24:06.549 &-57:46:17.23\\
shell &10:24:29.716 &-57:48:12.36\\
pillar &10:24:11.681  &-57:49:05.98\\
p1 & 10:23:56.185& -57:43:22.65\\
p3 & 10:24:30.308&-57:45:02.46 \\
p7 & 10:24:11.139&-57:40:32.25 \\
\enddata
\tablecomments{The positions correspond to the lines-of-sight along which the spectra are presented in Fig.~\ref{fig:spectra}.}
\label{tab:regions-pos}
\end{deluxetable}
%\end{rotatetable}

==> table1-old.tex <==
 

\begin{table*}
%\tiny
% \begin{adjustwidth}{-0.8cm}{}

\centering
\begin{threeparttable}
\caption{Observed and model intensity values in different regions of RCW~49 .}
\begin{tabular}{l c c c c c c c c c}
\hline\hline
\noalign{\smallskip}
& units & northern cloud & ridge & shell & pillar & p1 & p3 & p7 \\
  \hline
 \noalign{\smallskip}


& & 6.7  & 9.9   & 9.4   & 1.1   & 3.0   & 34.0   & 4.2  \\

$I$(\cii\,) & 10$^{-4}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$ & & & & & & 20.0   & \\

& & & & & & &12.0  & \\

\hline

& & 3.2  & 2.9  & 1.7  & 1.7  & 2.8  & 7.6 & 1.4 \\

$I$($^{12}$CO (3-2)) & 10$^{-6}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$  &  & & & & & 4.7 & \\

& & & & & & & 2.9 & \\

\hline

& & 0.37 & 3.0  & 2.0  & 1.8  & 0.33  & 11.0  & 0.5 \\

$I$(\oi\,) & 10$^{-3}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$ & & & & & & 1.3  & \\

& & & & & & & 1.5 & \\

\hline

$I$(H$_2$ 0-0 S(1)) & 10$^{-4}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$& & & & & 0.31 & 1.6  & 1.0  \\ 

\hline

$I$(H$_2$ 0-0 S(2)) & 10$^{-4}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$ & & & & & 0.75  & 2.2  & 1.2  \\

\hline

$I$(FIR)& erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$& 0.24 & 1.22 & 0.82 & 0.57 & 0.42 & 1.24 & 0.38 \\

\hline

& & 4.0  & 6.2  & 5.5  & 4.6 & 6.6  & 5.9  & 10.0 \\

$I_{\rm exp}$(\cii\,) & 10$^{-4}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$ & & & & & & 4.7 & \\

& & & & & & & 5.6 & \\
\hline 

& & 2.3  & 2.1  & 1.1  & 0.82  & 3.9  & 1.4  & 3.1  \\

$I_{\rm exp}$($^{12}$CO(3-2)) & 10$^{-6}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$& & & & & & 1.3  & \\

& & & & & & & 1.4  & \\

\hline


& & 1.1 & 2.4  & 1.4 & 0.87 & 6.74  & 1.7 & 11.0 \\

$I_{\rm exp}$(\oi\,) & 10$^{-3}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$& & & & & &  1.1 & \\

& & & & & & &  1.7 & \\

\hline

$I_{\rm exp}$(H$_2$ 0-0 S(1)) & 10$^{-5}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$ &  & & & & 7.9  & 3.4 & 22.0 \\

\hline

$I_{\rm exp}$(H$_2$ 0-0 S(2)) & 10$^{-5}$ erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$  &  & & & & 1.6  & 0.22 & 7.5  \\

 
 \hline
\end{tabular}
Notes: $I$ and $I_{\rm exp}$ are the observed and intensities predicted by models, respectively, in units of erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$. The three rows for p3 correspond to the intensities integrated over the entire velocity window of -30 to 30~km~s$^{-1}$, intensities integrated over the velocity window of -15 to 5~km~s$^{-1}$ and intensities integrated over the velocity window of 5 to 20~km~s$^{-1}$.

%\begin{tablenotes}
%\item[a]\small values are in units of erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$.

%\end{tablenotes}

 \label{tab:int-exp}
 \end{threeparttable}
% \end{adjustwidth}
% \end{sidewaystable*}
\end{table*}


==> table1.tex <==


\begin{deluxetable*}{l c c c c c c c c c c c c}
%\tabletypesize{\footnotesize}
%\tablecolumns{8}
%\tablewidth{\textwidth}
\tablecaption{\textbf{Observed and model intensity$^*$ values in different regions of RCW~49.}}
\label{tab:int-exp}
\tablehead{
 \colhead{Parameter} & 
% \colhead{Units} & 
 \colhead{rms noise} &
 \colhead{northern cloud} & 
 \colhead{ridge} & 
 \colhead{shell} & 
 \colhead{pillar} & 
 \colhead{p1} &
 \colhead{p3} & 
 \colhead{p3v1} &
 \colhead{p3v2} &
 \colhead{p7}
}

\startdata
{R.A. (J2000)} & & 10:23:59.7 &10:24:06.5 &  10:24:29.7 & 10:24:11.7 & 10:23:56.2 & 10:24:30.3 & & & 10:24:11.1\\
{Dec. (J2000)} & & -57:38:52.7 & -57:46:17.2&-57:48:12.4   &-57:49:06  &-57:43:22.7  &-57:45:02.5  & & & -57:40:32.3\\
 {$I$(\cii\,)} & 0.18 & 6.7  & 9.9   & 9.4   & 11.0   & 3.0   & 34.0 &20.0 &12.0   & 4.2\\
 {$I$($^{12}$CO (3-2))} & 0.003 & 0.032  & 0.029   & 0.017   & 0.017   & 0.028   & 0.076 & 0.047 & 0.029 & 0.014\\
 {$I$(\oi\,)}  &3.3 & 3.7  & 30.0   & 20.0   & 18.0   & 3.3   & 110.0 & 13.0 & 15.0 & 14.0\\
  {$I$(H$_2$ 0-0 S(1))} & 0.05 & & & & & 0.31 & 1.6  & & & 1.0  \\ 
{$I$(H$_2$ 0-0 S(2))} & 0.06 & & & & & 0.75  & 2.2  & & &1.2  \\
{$I$(FIR)}& & 2400 & 12200 & 8200 & 5700 & 4200 & 12400 & & &3800 \\
{$I_{\rm pre}$(\cii\,)} &  & 4.0 & 6.2 & 5.5 & 4.6 & 6.6 & 5.9 & 4.7& 5.6& 10.0 \\
{$I_{\rm pre}$($^{12}$CO (3-2))} &  & 0.023 & 0.021 & 0.011 & 0.0082 & 0.039 & 0.014 & 0.013& 0.014& 0.031 \\
{$I_{\rm pre}$(\oi\,)} &  & 11.0 & 24 & 14 & 8.7 & 67.4 & 17 & 11& 17& 110 \\
{$I_{\rm pre}$(H$_2$ 0-0 S(1))} &  & & & & & 0.79  & 0.34  & & &0.220  \\
{$I_{\rm pre}$(H$_2$ 0-0 S(2))} & & & & & & 0.16  & 0.022  & & &0.75  \\
\enddata
\tablecomments{\textbf{* All intensities are in the units of 10$^{-4}$ erg cm$^{-2}$ s$^{-1}$ sr$^{-1}$. The observed intensities were converted from K~km~s$^{-1}$ ($W$) to erg~cm$^{-2}$~s$^{-1}$~sr$^{-1}$ ($I$). 
For \cii\,~158~$\mu$m, $^{12}$CO (3--2) and \oi\,~63~$\mu$m, respectively, the conversions are $I$ (erg~s$^{-1}$~cm$^{-2}$~sr$^{-1}$) = 7.05 $\times$ 10$^{-6}$ $W$ (K~km~s$^{-1}$), 4.238 $\times$ 10$^{-8}$ $W$ (K~km~s$^{-1}$) and 1.1 $\times$ 10$^{-4}$ $W$ (K~km~s$^{-1}$).
$I$ and $I_{\rm pre}$ are the observed intensities and intensities predicted by models, respectively. The columns p3, p3v1 and p3v2 correspond to the intensities integrated over the velocity window of -30 to 30~km~s$^{-1}$, -15 to 5~km~s$^{-1}$ and 5 to 20~km~s$^{-1}$, respectively.
}}
\label{tab:int-exp}
\end{deluxetable*}
%\end{rotatetable}

%& -57:38:52.74

==> table2-new.tex <==
%\begin{rotatetable}
\begin{deluxetable*}{l c c c c c c c c c c}
%\tabletypesize{\footnotesize}
%\tablecolumns{8}
%\tablewidth{\textwidth}
\tablecaption{\textbf{Derived physical parameters in different regions of RCW~49.}}
\label{tab:phys-val-mwp}
\tablehead{
 \colhead{Parameter} & 
 \colhead{units} & 
 \colhead{northern cloud} & 
 \colhead{ridge} & 
 \colhead{shell} & 
 \colhead{pillar} & 
 \colhead{p1} &
 \colhead{p3} & 
 \colhead{p3v1} & 
 \colhead{p3v2} & 
 \colhead{p7}
}
\startdata
% {$n$(LSQ)} & 10$^3$~cm$^{-3}$ & 8.5(2.9) & 6.4(0.9)  & 3.0(0.1)  & 2.1(0.02)  & 26.0(20.0) & 4.3(0.8) & 3.6(0.9) &4.4(1.0) &14.0(11.0) \\
{$n$} & 10$^3$~cm$^{-3}$ & 8.6(0.5) & 6.4(0.35)  & 3.1(0.2)  & 2.2(0.1)  & 27.0(2.0) & 4.3(0.1) & 3.6(0.1) &4.5(0.2) &14.0(1.0) \\
{$G_{\rm 0}$} & 10$^3$ Habing units & 0.5(0.07) & 2.4(0.3) & 1.9(0.4) & 0.97(0.21) & 2.9(0.32) & 2.1(0.2) & 0.79(0.07) & 2.0(0.2) &32.0(8.0)\\
{$G_{\rm 0}$(FIR)} & 10$^3$ Habing units& 0.92 & 4.7 & 3.2 & 2.2  & 1.7  & 4.8 & & & 1.5 \\
{$T_{\rm surf}$} & K & 160 & 246 & 250 & 223 & 244 & 242 & 196 & 242 & 441 \\
$T_{\rm ex}$(\cii\,) & K & 55.2 & 72.0 &47.3&54.6&33.6& &70.4&73.0&36.8\\
$p_{\rm th}$ & $10^6$ K~cm$^{-3}$ & 1.4 & 1.6 & 0.77 & 0.5 & 6.6 & 1.0 & 0.71 &1.1 & 6.2\\
$p_{\rm turb}$ & $10^6$ K~cm$^{-3}$ & 9.4 & 3.0 & 3.5 & 1.8 & 25.0 & 12.0 & 3.9 &1.8 &19.0\\
$\Delta v^2_{\rm turb}$ & km$^2$~s$^{-2}$ & 38.5 & 16.7 & 39.9 & 29.3 & 32.1 & 101.4 & 38.1 &14.2 &48.4\\
$N_{\rm H}$ (160~$\mu$m) & 10$^{22}$~cm$^{-2}$ & 4.5 &3.3 &5.6 &4.2 &4.5 & &13.0 & 13.0 & 4.6\\
$N_{\rm H}$ ($^{13}$CO) & 10$^{22}$~cm$^{-2}$ & 1.3 &0.84 &0.36 &0.78 &1.3 & &1.6 & 1.3 & 0.4\\
\enddata
\tablecomments{\textbf{$n$ is hydrogen volume density and $G_{\rm 0}$ is far-UV flux determined from the PDR ToolBox. %LSQ indicates parameters estimated through least squares fit method and MCMC indicates estimation through Markov Chain Monte Carlo method. 
Errors from fits are in parenthesis. $G_{\rm 0}$ (FIR) is the far-UV flux determined from the Herschel data. $T_{\rm ex}$(\cii\,) is the \cii\ excitation temperature. $p_{\rm th}$ and $p_{\rm turb}$ are the thermal and turbulent pressures. $\Delta v^2_{\rm turb}$ is the turbulent velocity in km$^2$~s$^{-2}$. $N_{\rm H}$ (160~$\mu$m) and $N_{\rm H}$ ($^{13}$CO) are hydrogen column densities estimated using the 160~$\mu$m Herschel data and the $^{13}$CO APEX data. The columns p3, p3v1 and p3v2 correspond to the intensities integrated over the velocity window of -30 to 30~km~s$^{-1}$, -15 to 5~km~s$^{-1}$ and 5 to 20~km~s$^{-1}$, respectively.}}
\label{tab:phys-val}
\end{deluxetable*}
%\end{rotatetable}

==> table2.tex <==
%\begin{rotatetable}
\begin{deluxetable*}{l c c c c c c c}
%\tabletypesize{\footnotesize}
%\tablecolumns{8}
%\tablewidth{\textwidth}
\tablecaption{Derived physical parameters in different regions of RCW~49}
\label{tab:phys-val-mwp}
\tablehead{
 \colhead{Parameter} & 
 \colhead{northern cloud} & 
 \colhead{ridge} & 
 \colhead{shell} & 
 \colhead{pillar} & 
 \colhead{p1} &
 \colhead{p3} & 
 \colhead{p7}
}

\startdata
 {$n$(LSQ)} & 8.5(2.9) $\times 10^3$ &
  $6.4(0.9) \times 10^3$ &
  $3.0(0.1) \times 10^3$ &
  $2.1(0.02) \times 10^3$ &
  $2.6(2.0) \times 10^4$ &
  $4.3(0.8) \times 10^3$ &
  $1.4(1.1) \times 10^4$ \\
  & & & & & & 3.6(0.9) $\times 10^3$ & \\
  & & & & & & 4.4(1.0) $\times 10^3$ & \\
{$n$(MCMC)} & 8.6(0.5) $\times 10^3$ & 
 $6.4(0.35) \times 10^3$ &
 $3.1(0.2) \times 10^3$ &
 $2.2(0.1) \times 10^3$ &
 $2.7(0.2) \times 10^4$ &
 $4.3(0.1) \times 10^3$ &
 $1.4(0.1) \times 10^4$\\
 & & & & & & $3.6(0.1) \times 10^3$ & \\
 & & & & & & $4.5(0.2) \times 10^3$ & \\
{$G_{\rm 0}$(LSQ)} & 5.0(4.4)  $\times 10^2$ &
$2.4(1.1) \times 10^3$ &
$1.8(0.3) \times 10^3$ &
$9.0(0.3) \times 10^2$ &
$2.8(3.4) \times 10^3$ &
$2.1(1.9) \times 10^3$ &
$3.2(6.9) \times 10^4$\\
 & & & & & & $7.8(7.1) \times 10^2$ & \\
 & & & & & & $1.9(1.6) \times 10^3$ & \\
$G_{\rm 0}$(MCMC) &$ 5.0(0.7) \times 10^2$ &
$2.4(0.3) \times 10^3$ &
$1.9(0.4) \times 10^3$ &
$9.7(2.1) \times 10^2$ &
$2.9(3.2) \times 10^3$ &
$2.1(0.2) \times 10^3$ &
$3.2(0.8) \times 10^4$\\
 & & & & & &$ 7.9(0.7) \times 10^2$ & \\
 & & & & & & $2.0(0.2)\times 10^3$ & \\ 
$G_{\rm 0}$(FIR) & $9.2 \times 10^2$ &
$4.7 \times 10^{3}$ &
$3.2 \times 10^{3}$ &
$2.2 \times 10^{3}$ &
$1.7 \times 10^{3}$ &
$4.8 \times 10^{3}$ &
$1.5 \times 10^{3}$\\
$T_{\rm surf}$ & 160 &246 & 250 & 223 & 244 & 242 & 441 \\ 
 & & & & & & 196 & \\
 & & & & & & 242 & \\
{$T_{\rm ex}(\cii\,)$} & 55.2 &72.0 & 47.3 & 54.6 & 33.6 &   & 36.8 \\
 & & & & & & 70.4 & \\
 & & & & & & 73.0 & \\
$p_{\rm th}$  & $1.4 \times 10^{6}$ &
$1.6 \times 10^{6}$ &
$7.7 \times 10^{5}$ &
$5.0 \times 10^{5}$ &
$6.6 \times 10^{6}$ &
$1.0 \times 10^{6}$ &
$6.2 \times 10^{6}$\\
& & & & & & 7.1 $\times$ 10$^{5}$& \\
& & & & & &1.1 $\times$ 10$^{6}$  & \\
$p_{\rm turb}$ & $9.4 \times 10^{6}$ &
$3.0 \times 10^{6}$ &
$3.5 \times 10^{6}$ &
$1.8 \times 10^{6}$ &
$2.5 \times 10^{7}$ &
$1.2 \times 10^{7}$ &
$1.9 \times 10^{7}$\\
& & & & & & 3.9 $\times$ 10$^{6}$ & \\
& & & & & & 1.8 $\times$ 10$^{6}$ & 
\enddata
\tablecomments{$n$ is hydrogen volume density in units of cm$^{-3}$; $G_{\rm 0}$ is far-UV flux in Habing units. LSQ indicates parameters estimated through least squares fit method and MCMC indicates estimation through Markov Chain Monte Carlo method. Errors from fits are in parenthesis. $T_{\rm surface}$ is the model gas temperature (in units of K) at
$A_{\rm v}$ = 0.01 and is characteristic of the \cii\ and \oi\ emitting region. $T_{\rm ex}$(\cii\,) is the \cii\ excitation temperature in units of K. $p_{\rm th}$ and $p_{\rm turb}$ are the thermal and turbulent pressures in units of K~cm$^{-3}$. The three rows for p3 correspond to the physical parameters determined using intensities integrated over the entire velocity window of -30 to 30~km~s$^{-1}$, intensities integrated over the velocity window of -15 to 5~km~s$^{-1}$ and intensities integrated over the velocity window of 5 to 20~km~s$^{-1}$.}
\label{tab:phys-val}
\end{deluxetable*}
%\end{rotatetable}

==> table3-new.tex <==
%\begin{rotatetable}
\begin{deluxetable*}{l c c c c c c c c c}
%\tabletypesize{\footnotesize}
%\tablecolumns{8}
%\tablewidth{\textwidth}
\tablecaption{\textbf{Physical conditions estimated by phase-space diagrams.}}
\label{tab:phys-val-ph-sp}
\tablehead{
 \colhead{Parameter} & 
 \colhead{units} & 
 \colhead{northern cloud} & 
 \colhead{ridge} & 
 \colhead{shell} & 
 \colhead{pillar} & 
 \colhead{p1} &
% \colhead{p3} & 
 \colhead{p3v1} & 
 \colhead{p3v2} & 
 \colhead{p7}
}
\startdata
{$n$} (\cii\,-CO-FIR) & 10$^3$~cm$^{-3}$ & 5-10  & 1-100 & 0.5-5 & 1-100  &10-100  & 1-10&1-10  &1-10  \\
{$n$} (\cii\,-\oi\,-FIR) & 10$^3$~cm$^{-3}$ & 5-7 & 1-10  &  1-10 &  1-100 &0.1-1  & 0.5-5 & 0.5-5 & 0.1-70  \\
{$G_{\rm 0}$} (\cii\,-CO-FIR) & 10$^3$ Habing units & 0.5-0.7 & 1-50 & 0.5-1 & 1-10&0.8-6  &0.6-0.7 &1  & 0.7-1 \\
{$G_{\rm 0}$} (\cii\,-\oi\,-FIR) & 10$^3$ Habing units &  0.5-0.7  &  3-10&1 &0.7-10 & 1-4 &0.6-1 & 1 & 1 \\
\enddata
\tablecomments{\textbf{Parameters with \cii\,-CO-FIR correspond to the values estimated from the left panels of Figs.~\ref{fig:ph-sp-regs} and \ref{fig:ph-sp-spit-pos}. Similarly, parameters with \cii\,-\oi\,-FIR correspond to the values estimated from the right panels of Figs.~\ref{fig:ph-sp-regs} and \ref{fig:ph-sp-spit-pos}. }}
\label{tab:phys-val-ph-sp}
\end{deluxetable*}
%\end{rotatetable}

==> table3-old.tex <==

\begin{table}
 \begin{adjustwidth}{-0.4cm}{}
\small
%\left
\begin{threeparttable}
\caption{Hydrogen nucleus column densities in different regions of RCW~49.}
\begin{tabular}{l c c}
\hline\hline
\noalign{\smallskip}
Region & $N_{\rm H}$ (160~$\mu$m)  & $N_{\rm H}$ ($^{13}$CO) \\
 & (cm$^{-2}$)& (cm$^{-2}$)\\
  \hline
 \noalign{\smallskip}

northern cloud & 4.5 $\times$ 10$^{22}$& 1.3 $\times$ 10$^{22}$\\
ridge & 3.3 $\times$ 10$^{22}$& 8.4 $\times$ 10$^{21}$\\
shell & 5.6 $\times$ 10$^{22}$& 3.6 $\times$ 10$^{21}$\\
pillar & 4.2 $\times$ 10$^{22}$& 7.8 $\times$ 10$^{21}$\\
p1 & 4.5 $\times$ 10$^{22}$& 1.3 $\times$ 10$^{22}$\\
p3 (-15 to 5~km~s$^{-1}$) & 1.3 $\times$ 10$^{23}$& 1.6 $\times$ 10$^{22}$\\
p3 (5 to 20~km~s$^{-1}$) & 1.3 $\times$ 10$^{23}$& 1.3 $\times$ 10$^{22}$\\
p7 & 4.6 $\times$ 10$^{22}$& 4.0 $\times$ 10$^{21}$\\

\hline 
 
\end{tabular}

 \label{tab:colden}
 \end{threeparttable}
 \end{adjustwidth}
\end{table}
